Beamforming Tradeoff for Sensing and Communication in Cell-Free MIMO

This paper studies optimal joint beamforming (BF) for joint sensing and communication (JSAC) in small-scale cell-free MIMO (CF-MIMO) systems. While prior works have explored JSAC optimization using methods such as successive convex approximation (SCA) and semidefinite relaxation (SDR), many of these approaches either lack global optimality or require additional rank-reduction steps. In contrast, we propose an SDR-based optimization framework that guarantees globally optimal solutions without post-processing. To benchmark its performance, we introduce a standalone BF strategy that dedicates each access point (AP) exclusively to either communication or sensing. The proposed formulation builds upon a general multi-user system model, enabling future extensions beyond the single-user setting. Overall, our framework offers a globally optimal and computationally efficient BF design, providing valuable insights for the development of next-generation wireless networks.

==> ploten_test.tex <==
\begin{tikzpicture}[scale=0.8]
    \begin{axis}
    [
        xlabel={Communication $\mathrm{SNR}_{\mathrm{c}}$ [dB]},
        ylabel={Sensing $\mathrm{SNR}_{\mathrm{s}}$ [dB]},
        title={Achievable $(\mathrm{SNR}_{\mathrm{s}}, \mathrm{SNR}_{\mathrm{c}})$ Region for Sensing and Communication},
        xmin=0,
        ymin=0,
        grid=major,
        legend style={
            at={(0.3,0.3)},
            anchor=south,
            font=\scriptsize,
            cells={anchor=west},
            fill=none,
            draw=none
        }
    ]

    % 标注 alpha
    \node[anchor=south west] at (axis cs: 1.5, 11) { $\alpha = 0$};
    \draw[->,line width=0.25mm] (axis cs: 2, 12) -- (axis cs: 1, 13.3);  
    \node[anchor=north east] at (axis cs: 6, 1.8) { $\alpha = 1$};
    \draw[->,line width=0.25mm] (axis cs: 6, 1) -- (axis cs: 6.8, 2);  
% 蓝线绘图（不加 legend）
\addplot[color=blue, line width=2pt, forget plot]
    table [col sep=comma] {SNRregion.csv};
\addlegendimage{legend image code/.code={
  \draw[blue, line width=2pt] (0.2cm,0cm) -- (0.4cm,0cm);
}}
\addlegendentry{Achievable ($\mathrm{SNR}_{\mathrm{s}}, \mathrm{SNR}_{\mathrm{c}}$) Region}


    \addplot[color=Orange, only marks, mark=diamond*, mark size=3pt] table [col sep=comma] {SNR_points.csv};
    \addlegendentry{Optimal Trade-off Points}

    \addplot[color=Red, only marks, mark=*, mark size=3pt] table [col sep=comma] {SNRa.csv};
    \addlegendentry{MRT for Communication}

    \addplot[color=Cyan, only marks, mark=*, mark size=3pt] table [col sep=comma] {SNRb.csv};
    \addlegendentry{MRT for Sensing}

    \addplot[color=Purple, only marks, mark=square*, mark size=3pt] table [col sep=comma] {SNR_ZF.csv};
    \addlegendentry{Zero-Forcing BF}

    \addplot[color=Green, only marks, mark=triangle*, mark size=3pt] table [col sep=comma] {SNR_base.csv};
    \addlegendentry{Standalone BF}

    \end{axis}
\end{tikzpicture}

\caption{Performance comparison of different beamforming techniques for fixed channels. The channels are randomly generated as Gaussian-distributed vectors with dimension 3.}
\label{Ploten1}

